Mitigating Data Scarcity for Large Language Models

In recent years, pretrained neural language models (PNLMs) have taken the field of natural language processing by storm, achieving new benchmarks and state-of-the-art performances. These models often rely heavily on annotated data, which may not always be available. Data scarcity are commonly found in specialized domains, such as medical, or in low-resource languages that are underexplored by AI research. In this dissertation, we focus on mitigating data scarcity using data augmentation and neural ensemble learning techniques for neural language models. In both research directions, we implement neural network algorithms and evaluate their impact on assisting neural language models in downstream NLP tasks. Specifically, for data augmentation, we explore two techniques: 1) creating positive training data by moving an answer span around its original context and 2) using text simplification techniques to introduce a variety of writing styles to the original training data. Our results indicate that these simple and effective solutions improve the performance of neural language models considerably in low-resource NLP domains and tasks. For neural ensemble learning, we use a multilabel neural classifier to select the best prediction outcome from a variety of individual pretrained neural language models trained for a low-resource medical text simplification task.

==> helper.tex <==
\chapter{Helper}
\thispagestyle{fancy}
This is an example of a numbered section. You can also created unnumbered sections and subsections, although
I recommend against it. If you create unnumbered sections you will have to add them to the Table of Contents 
manually with the \texttt{addcontentsline} command. \footnote{By the way footnotes are a thing}.\\

\textit{Note: All titles (chapters, sections, subsections, etc must be in Title Case.)} 

\section*{An Unnumbered Section}
This is an unnumbered section that has not been added to the Table of Contents.

\subsection{Subsections!}
You can also create subsections. They follow the same rules as sections.


\section{Math Example}
This is a real short example of using the equation environment.

\begin{equation}
	y = mx + b
\end{equation}

There is an awful lot that the equation environment and math mode can do for you.


\section{References}
Here is an example of references using the natbib package. You can reference in a number of ways.  The
ones that are most useful are parenthetical \citep{xu2016optimizing,ahmad2020policyqa} or inline, as in \citet{bahdanau2014neural} 
said this or that. You can also include information within the citation \citep[e.g.][doesn't have any page numbers]{2003jgr}.  You don't even need to have the reference in your text to be included. \nocite{2004LPI}

You can also cite your references directly inline using the \texttt{bibentry} command as follows: \bibentry{article}


\section{Figures} \label{section:figures}
On the next page is a figure inclusion using the `graphicx' package. This puts figures on their own page by 
themselves. They don't need to be on separate pages, there is no requirement that they be on separate pages.
If you want to put a figure on a page with text, don't include the \emph{p!} option in square brackets at 
the begin figure command.

You can use most common file types with this package. Just make sure the file extension listed in the command
matches the actual file.

Also note that the \verb=\caption= command has an optional square-bracketed argument and a curly-bracketed 
argument.  Whatever you put in square brackets will be used as the short caption, and will go into the 
List of Figures.  The stuff in the curly brackets will be placed on the page under your figure.


\begin{figure}[p!]
\begin{center}
\includegraphics{figure.eps}
\caption[Short figure caption for LOF]{Sample figure caption (to appear below
the actual figure). \label{samplefig}}
\end{center}
\end{figure}

You can reference a figure later using the \verb=\label= command (Figure~\ref{samplefig}). This can also be
done for sections and chapters (Section~\ref{section:figures}).

\section{Big Files}
For big projects (like a thesis) it is sometimes helpful to separate your chapters indo different documents. This
can be done with the \verb=\input= command. Simply save your chapter as a separate .tex file without a header or
preamble, and then input it into the main dissertation file. Try to avoid using the \verb=\include= command as \LaTeX\
can get cranky with the formatting when ``including'' a .tex file.

\section{Non-Breaking Spaces}
The tilde character can be used to mark a non-breaking space. \LaTeX\ does a great job of lining words up, putting
in line breaks where appropriate, and making the text flow properly. However, there are some cases where you really
don't want \LaTeX\ to toss in a carriage return. The places that spring to mind are between numbers and their units,
and between Figure and Table references and their values. So for example, you don't want something like this in your
document:

\begin{quote}
	Blah blah blah blah blah blah blah blah blah is 10\\
	m from foo to bar.
\end{quote}

So always use the tilde when you use numbers with units, like 9.8~m~s$^{-2}$, and with references, like Figure~\ref{samplefig}.
This way \LaTeX\ will never put a line break between those elements.


\section{Hyperlinks}
You may have noticed a lot of blue text in this template. Those are internal hyperlinks that are automatically set up by 
the \texttt{hyperref} package. You can change the colors of the links by messing with the options in the preamble. For the
most part these links should set themselves up to work just fine by themselves. If you notice weird behavior you can usually
find solutions online. If not the use of the hyperlinks is purely for convenience when working with large documents and is not
required by the Grad College.

You can also use this package to include web links. Long links can sometimes escape the page margins though, so I recommend
giving them custom text: \href{https://grad.arizona.edu/gsas/dissertations-theses/dissertation-and-thesis-formatting-guides}
{A link to the UA Thesis guidelines.}

\section{Tables}
On the next page is a sample table, placed on the page by itself. Again, this table is pretty small, so it could 
probably just be placed on a page with text. To do this remove the \emph{p!} from the command. Working with tables in
\LaTeX\ is notoriously difficult, so make liberal use of StackExchange and Google. 

A comment on \texttt{deluxetable}. \texttt{deluxetable} is a special table package from the AAS formatting standards that
some people insist is much nicer than the default \LaTeX\ table. These people are wrong, and \texttt{deluxetable} is evil.
Therefore I have not included a way for this template to work with \texttt{deluxetable}. If you want to try, that's your
choice, but I cannot gurantee it won't break the template.

\begin{table}[p!]
\begin{center}
\caption[Short table caption for LOT]{Sample table caption (to appear with the actual table). \label{sampletable}}
\vspace{0.3in}
\begin{tabular}{ccc}
\hline 
\hline
Col A & Col B & Col C \\
\hline
1 & 2 & 3 \\
4 & 5 & 6\\
\hline
\end{tabular}
\end{center}
\end{table}

By the way, you can reference Tables like you can figures (Table~\ref{sampletable}).
